Entangling unitary gates on distant qubits with ancilla feedback

By using an ancilla qubit as a mediator, two distant qubits can undergo a non-local entangling unitary operation. This is desirable for when attempting to scale up or distribute quantum computation by combining fixed static local sets of qubits with ballistic mediators. Using a model driven by measurements on the ancilla, it is possible to generate a maximally entangling CZ gate while only having access to a less entangling gate between the pair qubits and the ancilla. However this results in a stochastic process of generating control phase rotation gates where the expected time for success does not correlate with the entangling power of the connection gate. We explore how one can use feedback into the preparation and measurement parameters of the ancilla to speed up the expected time to generate a CZ gate between a pair of separated qubits and to leverage stronger coupling strengths for faster times. Surprisingly, by choosing an appropriate strategy, control of a binary discrete parameter achieves comparable speed up to full continuous control of all degrees of freedom of the ancilla.

==> Entangling.tex <==
\relax 
\citation{GBQC}
\citation{RaussendorfBriegel}
\citation{QuantumComputationByAdiabaticEvolution}
\citation{KitaevAnyons}
\citation{ADQC}
\citation{ACQC}
\citation{QubusProposal}
\citation{ADQC,ACQC}
\citation{QuantumRegisterNVCentre,UlmNVCentreAncilla}
\citation{FlyingQubits}
\citation{OiDevittHollenberg}
\citation{RepeatUntilSuccessLinearOptics,DistributedQCCiracEkert}
\citation{BarrettKokHeralding}
\citation{RUSQCUsingStationaryAndFlyingQubits}
\newlabel{FirstPage}{{}{1}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {I}Background}{1}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {A}Introduction}{1}{}}
\citation{ParsimoniousAndRobust}
\citation{ADQC}
\citation{ADQC}
\citation{KHSOi01}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces An circuit diagram example of ancilla driven quantum computation using the connection interaction $(H_A\otimes H_R).CZ$ \cite  {ADQC}. The ancilla is prepared in a fixed state, the choice of measurement basis is represented by the application of the unitary gate $J(\beta )$ to the ancilla in order to draw attention to the symmetry between the action on the ancilla and the register.}}{2}{}}
\newlabel{fig:ADQCpaperSingleQubit}{{1}{2}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {B}Ancilla Driven Operations}{2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces A two qubit gate in the ADQC scheme, using the same connection interaction twice, enacts a deterministic entangling gate with probabilistic local unitary effects. Here, the choice of measurement basis is fixed.}}{2}{}}
\newlabel{fig:ADQCpaperTwoQubit}{{2}{2}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces A circuit for generating a two qubit control-unitary gate with an interaction parametrised by an arbitrary coupling strength $\alpha $: $\Delta _\alpha =e^{-i\alpha \sigma _z\otimes \sigma _z}$. Local gate differences on the ancilla can be accounted for by the setting of $U_i$, $U_a$ and $U_g$. Local gate effects on the register can by accounted by a measurement dependent post-correction $V_{1/2}$. $V_{1/2}$ will commute with $\Delta _\alpha $ thus several applications can be treated with a single post-correction.}}{2}{}}
\newlabel{fig:TwoQubitEntanglementCircuit}{{3}{2}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {II}Unguided behaviour of random generation}{3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces The distribution of the target region hitting times given by the simulation of the gate generation with an interaction with $\alpha =\frac  {\pi }{16}$. The mean hitting time is 74.1, the standard deviation is 74.5.}}{3}{}}
\newlabel{fig:HittingTimes}{{4}{3}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {III}Strategies for guided gate generation}{3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {A}The one step strategy}{4}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces The probability tree of the ``one step" strategy. The first step will always require generating a CZ equivalent gate, the other result will be dependent on the coupling and will then dictate all future conditions. The conditions are reset at each step with each new ancilla.}}{4}{}}
\newlabel{fig:ProbTree}{{5}{4}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces The final state of the ancilla can be seen as a mixture of four points on the Bloch sphere. In order for the post-measurement action to be unitary the four points must lie on a circle and the measurement basis axis go through the centre. The cap sizes dictate the probability of the results, the distribution of the points around the circle affects the entangling power of the gate generated. The result within the minor cap is the more likely but will generate a less entangling gate. By adapting the parameters $\beta $ and $\theta $ these two aspects can be controlled.}}{4}{}}
\newlabel{fig:BlochSpherePicture}{{6}{4}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {B}The ``flip-undo" strategy}{5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces The probability tree of the ``flip-undo" strategy receives all possible points in the strategy after 2 steps. After the first step, it can be seen as a repeat-until-success strategy where the time to repeat is 2 gate generations.}}{5}{}}
\newlabel{fig:FlipUndoTree}{{7}{5}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {IV}Numerical results}{6}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces A comparison of the unguided (dotted black) generation against the one step (solid red) and flip-undo (dashed blue) strategy with their expected hitting times against coupling strength. Relative to the unguided approach, the flip-undo strategy is nearly as completely effective as the one step strategy while required less ancilla control. The unguided expectation times are not well correlated with the coupling strength: while significant differences in step size from large coupling differences do impact on the number of steps, the ability to approach arbitrarily close to the target relates to the difference of the step size with rational divisions of $\pi $ making for small scale chaotic behaviour.}}{6}{}}
\newlabel{fig:ExpectationTimes}{{8}{6}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces A comparison of the one step (solid red) strategy against the flip-undo (dashed blue) strategy: the number of ancilla that need to be prepared to guarantee a 99.9\% chance of success.}}{6}{}}
\newlabel{fig:FlipUndoPlot}{{9}{6}{}{}{}}
\bibdata{bibliography}
\citation{ADQC}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces A comparison of strategies for different numbers of degrees of freedom at high coupling strengths. The solid red curve represents the 1 port/1 d.o.f. approach, the dotted black curve is the 2 port/ 1 d.o.f. strategy and the dashed blue curve is the 2 port/2 d.o.f. strategy. The threshold occurs at approximately $0.73\frac  {\pi }{4}$.}}{7}{}}
\newlabel{fig:PortStrategyComparison}{{10}{7}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces The maximum number of steps in a strategy as allowed by the hard limit of $\frac  {1}{p}$ for a given coupling, displayed over the top half of the range of coupling strengths.}}{7}{}}
\newlabel{fig:OneOverP}{{11}{7}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {V}Conclusion}{7}{}}
\bibstyle{unsrt}
\newlabel{LastPage}{{}{7}}

